Integrating Weakly Supervised Word Sense Disambiguation into Neural Machine Translation

This paper demonstrates that word sense disambiguation (WSD) can improve neural machine translation (NMT) by widening the source context considered when modeling the senses of potentially ambiguous words. We first introduce three adaptive clustering algorithms for WSD, based on k-means, Chinese restaurant processes, and random walks, which are then applied to large word contexts represented in a low-rank space and evaluated on SemEval shared-task data. We then learn word vectors jointly with sense vectors defined by our best WSD method, within a state-of-the-art NMT system. We show that the concatenation of these vectors, and the use of a sense selection mechanism based on the weighted average of sense vectors, outperforms several baselines including sense-aware ones. This is demonstrated by translation on five language pairs. The improvements are above one BLEU point over strong NMT baselines, +4% accuracy over all ambiguous nouns and verbs, or +20% when scored manually over several challenging words.

==> sections/comparison-with-yang.tex <==
Yang et al.\ \shortcite{yang2017multi} attempted adding sense information by using the weighted sense embeddings as input for neural MT. In details, they used the sense labels generated from a non-parametric skip-gram model \cite{arvind2014efficient}. For each input token, they computed the localization context vector by concatenating the output from last hidden states of an extra bi-direction RNN and used it to generate the correlated weight by comparing with each possible sense. Finally the directly used the weighted average sense embedding as the word embedding for encoder.

\begin{table*}[ht]
\centering
\begin{tabular}{l|l|l}
\hline
               & Yang et al \shortcite{yang2017multi}                        & Ours                     \\ \hline
sense label    & skip-gram                   & adaptive k-means       \\ \hline
context vector & localization                & aver. neighbour embed. \\ \hline
epoch max.     & 6                           & convergence (approx.15)                    \\ \hline
input embed.   & aver. weighted sense embed. & concatenation          \\ \hline
\end{tabular}
\caption{Difference between our model and Yang et al \protect\shortcite{yang2017multi}}
\label{tab:model_diff}
\end{table*}

Table \ref{tab:model_diff} shows the main differences between the 2 works. First, they use skip-gram model for sense labelling and we use our adaptive $k$-means clustering. Moreover, they build an additional bi-direction RNN and concatenate the vector generated from its hidden states as the context vector for each input token. While we compute the context vector by averaging the embeddings of its neighbour words. Finally, after generating the correlated weights for each listed sense by comparing it with the context vector, they use the average weighted sense embedding as the input vector to encoder but we use the concatenation vectors with both word embedding and the average weighted sense embedding.

In order to make a better comparison with their work, we represent the results of their model by using our English to French corpus in Table \ref{tab:yang_bleu}. And we will show our results with the same dataset in the next section.


\begin{table*}[ht]
\centering
\begin{tabular}{c|c|c|c|c}
\hline
\multirow{2}{*}{}      & \multicolumn{2}{c|}{Yang et al \shortcite{yang2017multi}} & \multicolumn{2}{c}{Yang et al \shortcite{yang2017multi} + convergence} \\ \cline{2-5} 
                       & random  & initialization  & random          & initialization  \\ \hline
\multirow{2}{*}{EN/FR} & 30.11   & 31.05 (-3.55)   & 33.77 (-0.83)   & 34.52 (-0.08)   \\ \cline{2-5} 
                       & \multicolumn{4}{c}{Baseline 34.60}                           \\ \hline
\end{tabular}
\caption{BLEU scores from Yang et al \protect\shortcite{yang2017multi}'s work with different settings comparison, along with EN/FR language pair using same dataset as our experiment.  ``initialization" means to initialize the sense embeddings generated from skip-gram while ``random" is to randomize the embeddings by NMT preprocessing}
\label{tab:yang_bleu}
\end{table*}


By comparing the result from Table \ref{tab:yang_bleu} and Table \ref{tab:bleu_all_result} based on the different matters shown in Table \ref{tab:model_diff}, we can conclude:
\begin{itemize}
\item For the WSD system, our adaptive $k$-means clustering performs better than skip-gram;
\item Localization, which they used for context vector calculation has less performance compare to averaging neighbour embeddings within the current sentence. Moreover, since for each input token needs to complete one extra bi-direction RNN for further sense weight calculation, it costs 3 times more for training process compare to our model.
\item Concatenating the word embedding and its correlated sense vector as input for encoder outperforms just use the sense embedding to represent each token. Since the encoder would not only get the sense information but also capture the information of the original word token itself.
\end{itemize}


